Lite DETR : An Interleaved Multi-Scale Encoder for Efficient DETR

Recent DEtection TRansformer-based (DETR) models have obtained remarkable performance. Its success cannot be achieved without the re-introduction of multi-scale feature fusion in the encoder. However, the excessively increased tokens in multi-scale features, especially for about 75\% of low-level features, are quite computationally inefficient, which hinders real applications of DETR models. In this paper, we present Lite DETR, a simple yet efficient end-to-end object detection framework that can effectively reduce the GFLOPs of the detection head by 60\% while keeping 99\% of the original performance. Specifically, we design an efficient encoder block to update high-level features (corresponding to small-resolution feature maps) and low-level features (corresponding to large-resolution feature maps) in an interleaved way. In addition, to better fuse cross-scale features, we develop a key-aware deformable attention to predict more reliable attention weights. Comprehensive experiments validate the effectiveness and efficiency of the proposed Lite DETR, and the efficient encoder strategy can generalize well across existing DETR-based models. The code will be available in \url{https://github.com/IDEA-Research/Lite-DETR}.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> resources/images/analyze_match.tex <==
\begin{figure*}[h]
\centering
\subfigure[The predicted mask of the $0$th layer of Mask2Former.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_ori_0.png}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[The predicted mask of the last layer of Mask2Former.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_ori_9.png}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[The predicted mask of the $0$th layer of Mask DINO.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_m2f_0.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[The predicted mask of the last layer of Mask2 DINO.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_m2f_9.png}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{(a)(b) are the $0$th and the last layer prediction of Mask2Former. Obviously the $2$ predictions of the same query are matched with different instances. (a) matches the rear vehicle and (b) matches the front vehicle.  (b)(c) shows those of our Mask DINO. The two predictions both match the front vehicle.}
\label{fig:analyze_match}
\end{figure*}


==> resources/images/reduction.tex <==
\begin{figure}[h]
%\centering
\includegraphics[width=1.05\linewidth]{resources/images/module.pdf}
\caption{Compression and extrication of low-level features. }
\label{fig:reduction1}
\end{figure}

==> resources/images/reduction1.tex <==
\begin{figure}[h]
% \vspace{-0.8cm}]
    \centering
    \includegraphics[width=1\textwidth]{resources/images/lightdetr.pdf}
    \caption{Compression and extrication of low-level features. }
    \label{fig:reduction1}
    % \vspace{-0.8cm}
\end{figure}

==> resources/tables/boxhelpmask.tex <==
% \begin{table}[h]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|c|c|ccccccc|c|c|c}
%     \midrule
%         \multicolumn{2}{c}{Tasks} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} &  \\
%          \scriptsize Box& \scriptsize Mask & & \\
%         \midrule
%         % Mask-RCNN & $400$ & Dense anchors  & $42.5$ & $48.2$ & $-$ & $-$ & $23.8$ & $45.0$ & $60.0$ & $207$ & $40$M & $21^{*}$ \\
%         % HTC \cite{chen2019hybrid}& $24$ & Dense anchors & $38.4$ & $42.3$ & $-$ & $-$ & $-$ & $-$ & $-$ &$441$ & $80$M & $5^{*}$ \\
%         % QueryInst &&&&&&&&&& \\
       
%         % \hline
       
        
%         % DINO-4scale    &36 & 900 queries & - &{50.5}& $-$ & $-$ & $-$ & $-$ & $-$&$279$ & $47$M & 24\\
%         % DINO-4scale    &36 & 300 queries & - &{49.6}& $-$ & $-$ & $-$ & $-$ & $-$ &$279$ & $47$M & 24\\
%         % \hline
%         % Mask2Former$^*$    &50 & 100 queries& {43.7} & 46.2$^{\dag}$ & $-$ & $-$ & $23.4$ & $47.2$ & $64.8$ &$226$ & $44$M & 9.7 \\
%         % Mask DINO    &50 & 100 queries  &{45.4} &{49.8} & $-$ & $-$ & $-$ & $-$ & $-$ &$-$ & $44$M & - \\
%         % Mask DINO    &50 & 300 queries  &\textbf{46.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.3)} &\textbf{50.5} & $68.9$ & $50.3$ & \textbf{26.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.6)} & $49.3$ & $65.5$ &$234$ & $44$M & - \\
%         %  \hline
%         % Mask2Former    &12 & 100 queries& {38.7} & -& $-$ & $-$ & $23.4$ & $47.2$ & $64.8$ &$226$ & $44$M & 9.7 \\
%         % Mask DINO    &12 & 300 queries  &\textbf{41.4}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.7)} &{44.5} & $-$ & $-$ & $-$ & $-$ & $-$ &$234$ & $44$M & - \\
%         \midrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for Mask DINO and other object detection and instance segmentation models with the ResNet-50 backbone on COCO \texttt{val2017}. We follow the common practice in DETR-like models to use 300 queries. $^*$ The performance of Mask2Former will degenerate when using 300 queries. $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:boxhelpmask}
%     % \vspace{-.4cm}
% \end{table}

==> resources/tables/compare.tex <==
\begin{table*}[t]
    \centering
        \footnotesize
            \renewcommand{\arraystretch}{1.3}
    % \resizebox{\columnwidth}{!}{%
    \begin{adjustbox}{width=.9\textwidth,center}
    \begin{tabular}{lccccccc}
        \hline
        Models              & Detection & Segmentation & End-to-End & Feature Extraction & Denoising & Box Helps Mask &  Mask Helps Box \\
        % object queries: learned embedding fixed for all layers
        % learned anchors dynamically update for each layer
        \hline
        Mask-RCNN~\cite{he2017mask}           & \checkmark & Instance &  & RoI pooling & No&\checkmark&\checkmark  \\
        DETR~\cite{carion2020end}                & \checkmark & Panoptic and instance    &  \checkmark   & Standard attention&No&\checkmark&\\
        DINO~\cite{zhang2022dino}    & \checkmark & No   &  \checkmark    & Deformable attention & Contrastive DN for box&&\\
        HTC~\cite{chen2019hybrid}         & \checkmark & Instance   &     & RoI pooling &  No     &\checkmark& \checkmark  \\
        Mask2former~\cite{cheng2021mask2former}         &  & Panoptic, instance, and semantic  & \checkmark  & Masked attention & No        \\
        Mask DINO (ours)          & \checkmark & Panoptic, instance, and semantic &  \checkmark   & Deformable attention & DN for both mask and box&\checkmark&\checkmark   \\
        \hline
    \end{tabular}
    \end{adjustbox}
    % }
    \caption{Comparison of representative related models and Mask DINO. 
    % The term ``Detection" and ``Segmentation" shows whether the model can do detection or segmentation task. 
    ``End-to-end" shows whether the model is end-to-end optimized without handcrafted components such as NMS. ``Feature extraction" shows how each model pools features. ``Denoising" indicates what kind of denoising scheme is used in DINO and Mask DINO, where DN stands for query denoising~\cite{li2022dn}. ``Box helps mask" and ``Mask helps box" show mutual task cooperation between the two tasks.
    % whether the box head helps learn masks and the mask head can help learn boxes.
    }
    \label{tab:related_works}
    \vspace{-.4cm}
    
\end{table*}

==> resources/tables/instance.tex <==
\begin{table*}[t]
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=1.0\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|c|c|cc|ccccc|c|c|c}
    \toprule
        Model  & Epochs & Query type &Mask AP &Box AP & AP$_{50}^{mask}$ & AP$_{75}^{mask}$ & AP$_{S}^{mask}$ & AP$_{M}^{mask}$ & AP$_{L}^{mask}$ & GFLOPS & Params&FPS \\
        \midrule
        % Mask-RCNN & $400$ & Dense anchors  & $42.5$ & $37.2$ & $-$ & $-$ & $23.8$ & $45.0$ & $60.0$ & $207$ & $40$M & $21^{*}$ \\
        Mask-RCNN~\cite{he2017mask,du2021simple,ghiasi2021simple}, & $400$ & Dense anchors  & $42.5$ & $48.2$ & $-$ & $-$ & $23.8$ & $45.0$ & $60.0$ & $207$ & $40$M & $10.3$ \\
        HTC \cite{chen2019hybrid}& $36$ & Dense anchors & $39.7$ & $44.9$ & $61.4$ & $43.1$ & $22.6$ & $42.2$ & $50.6$ &$441$ & $80$M & $5$ \\
        QueryInst~\cite{fang2021instances} &36&300 queries&$40.6$&$45.6$&$63.0$&$44.0$&$23.4$&$42.5$&$52.8$&$-$&$-$&$7.0$ \\
        \hline
        DINO-4scale~\cite{zhang2022dino}    &36 & 900 queries & $-$ &{50.7}& $-$ & $-$ & $-$ & $-$ & $-$&$245$ & $47$M & $19.6$\\
        DINO-4scale~\cite{zhang2022dino}   &36 & 300 queries & $-$ &{49.6}& $-$ & $-$ & $-$ & $-$ & $-$ &$236$ & $47$M & $21.0$\\
         \hline
        Mask2Former~\cite{cheng2021mask2former}    &12 & 100 queries& {38.7} & $-$& $59.8$ & $41.2$ & $18.2$ & $41.5$ & $59.8$ &$226$ & $44$M & $8.2$ \\
        Mask DINO (ours)    &12 & 300 queries  &\textbf{41.4}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.7)} &{45.7} & $62.9$ & $44.6$ & $21.1$ & $44.2$ & $61.4$ &$290$ & $52$M & $14.8$ \\
        \hline
         Mask DINO (ours)    &\textbf{24} & 300 queries  &\textbf{44.2}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.5)} &{48.4} & $66.6$ & $47.9$ & $23.9$ & $47.0$ & $64.0$ &$290$ & $52$M & $14.8$ \\
        \hline
        Mask2Former$^*$~\cite{cheng2021mask2former}    &50 & 100 queries& {43.7} & 46.2$^{\dag}$ & $66.0$ & $46.9$ & $23.4$ & $47.2$ & $64.8$ &$226$ & $44$M & 8.2 \\
        Mask DINO (ours)    &50 & 100 queries  &{45.4} &{49.8} & $67.9$ & $49.3$ & $25.2$ & $48.3$ & $65.8$ &$227$ & $50$M & $15.2$ \\
        Mask DINO (ours)    &52 & 300 queries  &\textbf{46.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.3)} &{50.5} & $68.9$ & $50.3$ & \textbf{26.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.6)} & $49.3$\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.1)} & $65.5$\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.7)} &$290$ & $52$M & $14.8$ \\
        \hline
        \begin{tabular}[l]{@{}l@{}}Mask DINO (ours) \\ +\emph{Mask-enhanced box initialization}\end{tabular}     &50 & 300 queries  &\textbf{46.3}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.6)} &\textbf{51.7}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.0)} & $69.0$ & $50.7$ & \textbf{26.1}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.7)} & $49.3$\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.1)} & $66.1$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.3)} &$290$ & $52$M & $14.2$ \\
        
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for Mask DINO and other object detection and instance segmentation models with a ResNet-50 backbone on COCO \texttt{val2017}. We follow the common practice in DETR-like models to use 300 queries. $^*$ Mask2Former using 300 queries is not listed as its performance will degenerate when using 300 queries. $^\dag$ indicates the box AP is derived from mask prediction. We test the FPS and GFLOPS of Mask2Former and Mask DINO on the A100 GPU using detectron2.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:instance}
    \vspace{-.4cm}
\end{table*}

==> resources/tables/main_ablation.tex <==
\begin{table*}[!t]
\begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{minipage}[t]{0.5\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{cccc}
%     \toprule
%     \multicolumn{2}{c}{Matching} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} \\
%           Box&  Mask & & \\
%         \midrule
%     \checkmark     &      & $44.4$ & $40.5$ \\
%      & \checkmark  & $40.2$ &$38.4$     \\
%     \checkmark & \checkmark     & $\textbf{44.5}$ & $\textbf{41.4}$      \\
%     \bottomrule
% \end{tabular}
% \caption{Matching method comparison on COCO Val under 12-epoch setting.}
% \label{sample-table}
% \end{minipage}
    \begin{minipage}[t]{0.48\textwidth}
\makeatletter\def\@captype{table}
\centering
\vspace{-45pt}
\begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c}{Matching} & \multirow{2}{*}{Box AP} & \multirow{2}{*}{Mask AP} \\
          Box&  Mask & & \\
        \midrule
    \checkmark     &      & $44.4$ & $40.5$ \\
     & \checkmark  & $40.2$ &$38.4$     \\
    \checkmark & \checkmark     & $\textbf{44.5}$ & $\textbf{41.4}$      \\
    \bottomrule
\end{tabular}
\caption{Matching method comparison under the 12-epoch setting. We train both tasks together but use different matching methods to verify the effectiveness of hybrid matching.}
\label{tab:match}
\end{minipage}\hspace{6mm}
\begin{minipage}[t]{0.85\textwidth}
\makeatletter\def\@captype{table}
\centering
    \begin{tabular}{l|ccc}
        \toprule
          & Box AP & Mask AP   \\
        \midrule
         Mask DINO (ours) & \textbf{45.7}&\textbf{41.4} \\
         \midrule
        %  $-$ DINO Mask branch$^*$  & 49.5$^{\dag}$&35.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-5.7)}   \\
        $-$ Mask-enhanced anchor box initialization  & 44.5\fontsize{7.0pt}{\baselineskip}\selectfont{(-1.2)}&41.4    \\
         \quad$-$ Unified query selection for masks  & 43.6\fontsize{7.0pt}{\baselineskip}\selectfont{(-2.1)} &40.3\fontsize{7.0pt}{\baselineskip}\selectfont{(-1.1)}   \\
        $-$ Unified denoising for masks & 44.4\fontsize{7.0pt}{\baselineskip}\selectfont{(-1.3)}&40.3 \fontsize{7.0pt}{\baselineskip}\selectfont{(-1.1)}    \\
        $-$ Hybrid matching & 44.9\fontsize{7.0pt}{\baselineskip}\selectfont{(-0.8)} & 40.5 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.9)}   \\
        \midrule
        $-$ remove all the above & 41.7 & 38.5 \fontsize{7.0pt}{\baselineskip}\selectfont{(-2.7)}   \\
        \bottomrule
    \end{tabular}
    \caption{Comparison of the proposed components under the 12-epoch setting. $^*$ indicates that we use the original DETR~\cite{carion2020end} segmentation branch in Mask DINO, where we follow DETR to fine-tune segmentation after finishing training detection. $^{\dag}$ the performance of detection drops ($49.6$ AP as shown in Table \ref{tab:instance} when only training detection) after training segmentation.
    }
    \label{tab:ablation}
    \end{minipage}
    \end{adjustbox}
    \vspace{-.5cm}
\end{table*}
    % \vspace{-.8cm}
% \end{table}
% \begin{table}[h]
% % \vspace{-0.4cm}
%     \centering
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cc|ccccccc}
%         \midrule
%         \#Row  & box AP & mask AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\
%         \midrule
%         1. Basic Mask DINO & Running \\
%         2. Row1 + Hybrid matching & Running   \\
%         % 1. Optimized DN-DETR &  No & & \checkmark  & $45.2$ & $61.6$ & $48.7$ & $27.2$ & $48.0$ & $59.6$\\
%         3. Row2 + Mask denoising & TODO 095    \\
%         % 3.  & Pure  &  & \checkmark  & $46.7$ & $63.9$ & $50.9$ & $29.8$ & $49.8$ & $61.3$\\
%         % 4. + Mask denoising & Mixed  &  &  & $47.0$ & $64.2$ & $51.0$ & $31.1$ & $50.1$ & $61.5$\\
%         % 4.  & Mixed  &  & \checkmark & $47.0$ & $65.1$ & $50.9$ & $28.9$ & $50.1$ & $62.0$\\
%         % 5. Row4+look forward twice  & Mixed  &  & \checkmark  & $47.4$ & $64.8$ & $51.6$ & $29.9$ & $50.8$ & $61.9$\\
%         4. {Mask DINO} (ours, Row3 + Unified query selection for masks)  & 44.5&41.4   \\
%         \midrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     \vspace{0.3cm}
%     \caption{Ablation comparison of the proposed algorithm components.
%     }
%     % \vspace{-0.1cm}
%     \label{tab:ablation}
%     \vspace{-.8cm}
% \end{table}

% \begin{minipage}[t]{0.4\textwidth}
% \makeatletter\def\@captype{table}
%     \begin{tabular}{cccccccccc}
%         \midrule
%           & box AP & mask AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\
%         \midrule
%          Mask DINO & 44.5&\textbf{41.4} \\
%          \midrule
%          $-$ DINO Mask branch$^*$  & 49.5$^{\dag}$&35.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-5.7)}   \\
%          $-$ Unified query selection for masks  & 43.6&40.3 \fontsize{7.0pt}{\baselineskip}\selectfont{(-1.1)}   \\
%          $-$ Hybrid matching & 44.4 & 40.5 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.9)}   \\
%         $-$ Mask denoising & 44.6&40.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.7)}    \\
%         \midrule
%     \end{tabular}
%     % \caption{Ablation comparison of the proposed components under 12-epoch setting on COCO val. $^*$ indicates we use original DETR~\cite{carion2020end} segmentation branch with $300$ queries, where we follow DETR to finetune segmentation after finishing training detection. $^{\dag}$ the performance of detection drops ($49.6$ AP as shown in Table \ref{tab:instance} when only training detection) after training segmentation.
%     % }
%     \label{tab:ablation}
%     \end{minipage}


==> resources/tables/panoptic.tex <==
\begin{table*}[t]
% \vspace{-.4cm}
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    % \resizebox{\textwidth}{!}{%
    \begin{adjustbox}{width=0.9\textwidth,center}
    % \begin{tabular}{l|c|cccccc}
    \begin{tabular}{l|c|c|ccc|ccc}
    \toprule
        Model  & Epochs & Query type &PQ &PQ$^{Th}$ & PQ$^{St}$ & Box AP$^{Th}_{pan}$ & Mask AP$^{Th}_{pan}$   \\
        \midrule
        DETR~\cite{carion2020end} & $500+25$ & 100 queries  & $43.4$ & $48.2$ & $36$ & $-$ & $31.1$\\% & $-$ \\
        Panoptic Segformer~\cite{li2021panoptic} & 24& 353 queries&$49.6$&$54.4$&$42.4$& $-$&$41.7$\\%& $-$ \\
        Mask2Former$^*$ \cite{cheng2021mask2former}   &50 & 100 queries& {51.9}/$51.5^\dag$ & 57.7 & $43.0$ & $-$ & $41.7$ \\%& $61.7$  \\
        
        % Mask DINO    &50 & 100 queries  &{45.4} &{49.8} & $-$ & $-$ & $-$ & $-$ & $-$ &$-$ & $44$M & - \\
        Mask DINO (ours)    &{50} & 100 queries  & $52.3$&$58.3$&$43.2$&$47.7$&$43.7$ \\%&$59.5$\\
        Mask DINO (ours)    &50 & 300 queries  &\textbf{53.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.1)} &\textbf{59.1}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.4)} & $\textbf{43.9}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.9)} & $\textbf{48.8}$ & \textbf{44.3}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.6)} \\%& $59.6$   \\
        Mask DINO (ours)    &\textbf{24} & 300 queries  & $51.5$ &$57.3$&$42.6$&$46.4$&$42.8$\\%&$58.3$ \\
         \hline        
        Mask2Former~\cite{cheng2021mask2former}    &12 & 100 queries& {46.9} & $52.5$ & $38.4$ & $-$ &  37.2\\%& $58.0$  \\
        Panoptic Segformer~\cite{li2021panoptic}&12&353 queries &$48.0$ & $52.3$ &$41.5$& $-$& $-$\\%& $-$\\
        Mask DINO (ours)    &12 & 300 queries  &\textbf{49.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.0)} &{54.8} & $40.2$ & $43.2$ & $\textbf{40.4}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+3.2)} \\%& $54.8$   \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    \centering
    % \vspace{0.2cm}
    \caption{Results for Mask DINO and other panoptic segmentation models with a ResNet-50 backbone on COCO \texttt{val2017}. $^*$ Mask2Former using 300 queries is not listed as its performance will degenerate
when using 300 queries. 
$^\dag$ Our reproduced result.
    % $\dag$ indicates the box AP is generated from mask prediction.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    \label{tab:panoptic}
    \vspace{-.4cm}
\end{table*}

==> resources/tables/scaleandlayernum.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=1.0\textwidth,center}
% \begin{minipage}[t]{0.58\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% \begin{tabular}{c|ccc}
%     \toprule
%   Feature scale & box AP & {mask AP} & FLOPs \\
%         \midrule
%     single scale(1/8)     &  $45.8$    & $45.1$  \\
%      3 scales  & $50.5$ & $45.8$   \\
%     4 scales & $50.5$ & $\textbf{46.0}$     \\
%     \bottomrule
% \end{tabular}
% \caption{Feature scales comparison for Transformer decoder on COCO val under 50-epoch setting with Resnet-50 backbone.}
% \label{tab:feature_scale}
% \end{minipage}\hspace{10mm}
% \begin{minipage}[t]{0.58\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% \begin{tabular}{c|ccc}
%     \toprule
%   Decoder layer\# & box AP & {mask AP} & FLOPs \\
%         \midrule
%         3&$43.1$&$40.7$\\
%      6     &$44.3$    & $41.1$  \\
%      9  &  $44.5$    & $\textbf{41.4}$  \\
%     12 & $44.8$ & $41.1$     \\
%     \bottomrule
% \end{tabular}
% \caption{Decoder layer number comparison on COCO Val under 12-epoch setting.}
% \label{tab:dec_layer}
% \end{minipage}
\begin{minipage}[t]{0.56\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c}{Tasks} & \multirow{2}{*}{Box AP} & \multirow{2}{*}{Mask AP} \\
          Box&  Mask & & \\
        \midrule
    \checkmark     &      & $50.1$ &- \\
     & \checkmark  & - & $43.3$   \\
    \checkmark     & \checkmark & $\textbf{50.5}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.4)} & $\textbf{46.0}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.7)}     \\
    \bottomrule
\end{tabular}
\caption{Task comparison under the 50-epoch setting. We train the same Mask DINO with different tasks and validate that box and mask can achieve mutual cooperation.}
\label{tab:taskhelp}
\end{minipage}\hspace{6mm}
\begin{minipage}[t]{0.9\textwidth}
\makeatletter\def\@captype{table}
\centering
\centering
\vspace{-37.005pt}
\begin{tabular}{c|c|ccccc}
    \toprule
    &Epochs& PQ & PQ$^{thing}$& PQ$^{stf}$&Box AP$^{Th}_{pan}$&Mask AP$^{Th}_{pan}$ \\
        \midrule
        w/o decouple&12&$47.9$&$54.0$&$38.8$&$42.8$&$39.6$\\
     w/ decouple    &12 &$\textbf{49.0}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.1)}    & $\textbf{54.8}$& $\textbf{40.2}$& $\textbf{43.2}$& $\textbf{40.4}$  \\
     \midrule
     w/o decouple  &50&  $52.7$  & $58.8$&$43.5$&$48.7$&$44.1$  \\
    w/ decouple &50 &\textbf{53.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.3)} &\textbf{59.1} & $\textbf{43.9}$ & $\textbf{48.8}$ & \textbf{44.3}     \\
    \bottomrule
\end{tabular}
\caption{Effectiveness of decoupled box prediction for panoptic segmentation under the 12-epoch and 50-epoch settings.}
\label{tab:decouple}
\end{minipage}
\end{adjustbox}
\vspace{-.4cm}
\end{table*}

% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{ccc}
%     \toprule
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
% \end{tabular}
% \caption{Sample table title}
% \label{sample-table}
% \end{minipage}
% \end{minipage}


==> resources/tables/semantic.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{minipage}[t]{0.7\textwidth}
\makeatletter\def\@captype{table}
\centering
\large
\begin{tabular}{c|cc|ccc}
    \toprule
        Model  & Iterations& \begin{tabular}[c]{@{}c@{}}Crop\\ size\end{tabular}&\begin{tabular}[c]{@{}c@{}}mIoU\\(mean)\end{tabular} &\begin{tabular}[c]{@{}c@{}}mIoU\\(high)\end{tabular}&\begin{tabular}[c]{@{}c@{}}mIoU\\(reported)\end{tabular}  \\
        \midrule
        Mask2Former~\cite{cheng2021mask2former} &160k& $512$&$46.1$ & $46.5$ &$47.2$  \\
          Mask DINO (ours)    & 160k& $512$&$\textbf{47.7}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.6)} &\textbf{48.7}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.2)}&\textbf{48.7}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.6)}\\  \bottomrule
    \end{tabular}
    \centering
    \captionsetup{font={large}}
    \caption{{Results for Mask DINO and Mask2Former with 100 queries using a ResNet-50 backbone on ADE20K \texttt{val}. 
    % $^*$The reported performance in \cite{cheng2021mask2former} is $47.2$. 
    We found the performance variance on this dataset is high and run three times to report both the mean and highest results for both models}.
    }
    \label{tab:sematic_ade}
\end{minipage}\hspace{10mm}
\begin{minipage}[t]{0.7\textwidth}
\makeatletter\def\@captype{table}
\centering
\large
\begin{tabular}{c|c|cccc}
    \toprule
        Model  & Iterations &\begin{tabular}[c]{@{}c@{}}mIoU\\(mean)\end{tabular} &\begin{tabular}[c]{@{}c@{}}mIoU\\(high)\end{tabular}&\begin{tabular}[c]{@{}c@{}}mIoU\\(reported)\end{tabular}  \\
        \midrule
        Mask2Former~\cite{cheng2021mask2former} &90k&$78.7$ & $79.0$&$79.4$   \\
          Mask DINO (ours)   & 90k &\textbf{79.8}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.1)} &\textbf{80.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.0)}&\textbf{80.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.6)}  \\
    \bottomrule
    \end{tabular}
    \centering
    % \vspace{0.2cm}
    \captionsetup{font={large}}
    \caption{Results for Mask DINO and Mask2Former with 100 queries using a ResNet-50 backbone on Cityscapes \texttt{val}. 
    % $^*$The reported performance in \cite{cheng2021mask2former} is $79.4$. 
    We found the performance variance on this dataset is high and run three times to report both the mean and highest results for both models.
    }
    \label{tab:sematic_c}
\end{minipage}
\end{adjustbox}
\vspace{-0.4cm}
\end{table*}

% \begin{table}[h]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=.5\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{c|cc|ccc}
%     \midrule
%         Model  & Iterations& Crop size &mIoU (s.s.)  \\
%         \midrule
%         Mask2Former &160k& $512$ & $47.2$   \\
%           Mask DINO   & 160k&$512$  &\textbf{48.7}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.5)}  
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for Mask DINO and other semantic segmentation models with the ResNet-50 backbone on ADE20K \texttt{val}.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:sematic}
%     % \vspace{-.4cm}
% \end{table}

==> resources/tables/sota.tex <==
\begin{table*}[t]
    \centering
    \small
        \setlength\tabcolsep{2pt}
        \footnotesize
            \renewcommand{\arraystretch}{1.3}
    % \resizebox{}{!}{%
    % \resizebox{0.5\columnwidth}{!}{%
    % \resizebox{\columnwidth}{!}
    \begin{adjustbox}{width=0.7\textwidth,center}
    \begin{tabular}{c|c|c|c|c|cc}
    % \begin{tabular}{c|c|c|c|c|c|c|ccc}
        \toprule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Params} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{\makecell{Backbone Pre-training \\ Dataset }} &  \multirow{2}{*}{\makecell{Detection Pre-training \\ Dataset }}   & \multicolumn{2}{c}{{ val}}  \\
        & & &  && \scriptsize w/o TTA& \scriptsize w/ TTA  \\
        \midrule
        \multicolumn{5}{c}{{\textbf{Instance segmentation on COCO}}}&\multicolumn{2}{c}{AP} \\
        \midrule
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
        Mask2Former~\cite{cheng2021mask2former} & $216$M & SwinL & IN-22K-14M & $-$    & $50.1$ & $-$  \\
        Soft Teacher~\cite{xu2021end} & $284$M & SwinL & IN-22K-14M & O365     &$51.9$ & $52.5$  \\
        SwinV2-G-HTC++~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & O365    & $53.4$ & $53.7$ \\
        \hline
        MasK DINO(Ours) & $\textbf{223}${M} & SwinL & IN-22K-14M & - &    $\textbf{52.6}$ & ${-}$  \\
        % \hline
        MasK DINO(Ours) & $\textbf{223}${M} & SwinL & IN-22K-14M & O365 &    $\textbf{54.5}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.1)} & ${-}$  \\
        
        \midrule
        \multicolumn{5}{c}{{\textbf{Panoptic segmentation on COCO}}}&\multicolumn{2}{c}{PQ} \\
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
       
        Panoptic SegFormer~\cite{li2021panoptic}& $-$M & SwinL & IN-22K-14M & $-$     &$55.8$ & $-$  \\
         Mask2Former~\cite{cheng2021mask2former} & $216$M & SwinL & IN-22K-14M & $-$     & $57.8$ & $-$  \\
        % SwinV2-G~\cite{liu2021swinv2} & $3.0$B & IN-22K-ext-70M~\cite{liu2021swinv2} & O365 &   & $61.9$ & $62.5$ & $-$ & $63.1$\\
        \hline
        MasK DINO (ours) & ${223}${M} & SwinL & IN-22K-14M &  &    $\textbf{58.4}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.6)} & ${-}$  \\
        % \hline
        MasK DINO (ours) & ${223}${M} & SwinL & IN-22K-14M & O365 &    $\textbf{59.4}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.6)} & ${-}$  \\
        \midrule
        \multicolumn{5}{c}{{\textbf{Semantic segmentation on ADE20K}}}&\multicolumn{2}{c}{mIoU} \\
        \midrule
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
        Mask2Former~\cite{cheng2021mask2former} & $215$M & SwinL & IN-22K-14M  & $-$     & $56.1$ & $57.3$  \\
        % Mask2Former~\cite{cheng2021mask2former} & $217$M & SwinL-FaPN & IN-22K-14M  & $-$     & $56.4$ & $57.7$   \\
        SeMask-L MSFaPN-Mask2Former~\cite{jain2021semask} & $-$M & SwinL-FaPN & IN-22K-14M & $-$     &$-$ & $58.2$  \\
        SwinV2-G-UperNet~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & $-$ &   $59.3$ & $59.9$\\
        \hline
        MasK DINO (ours) & $\textbf{223}$\textbf{M} & SwinL & IN-22K-14M & $-$ &    $\textbf{56.6}$ & $\textbf{-}$  \\
        MasK DINO (ours) & $\textbf{223}$\textbf{M} & SwinL & IN-22K-14M & O365 &    $\textbf{59.5}$ & $\textbf{60.8}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.9)}  \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % }
    % \vspace{0.05cm}
    \caption{Comparison of the SOTA models on three segmentation tasks. Mask DINO outperforms all existing models. "TTA" means test-time-augmentation.
    % Similar to DETR~\cite{carion2020end}, we use the term ``end-to-end'' to indicate if a model is free from hand-crafted components like RPN and NMS.
    ``O365''  denotes the  Objects365~\cite{shao2019objects365} dataset. 
    }
    \label{tab:sota}
    \vspace{-.3cm}
\end{table*}

% \begin{table}
% % \vspace{-0.4cm}
%     \centering
%     \small
%         \setlength\tabcolsep{2pt}
%         \footnotesize
%             \renewcommand{\arraystretch}{1.3}
%     % \resizebox{}{!}{%
%     % \resizebox{0.5\columnwidth}{!}{%
%     % \resizebox{\columnwidth}{!}
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{c|c|c|c|c|cc|cc}
%     % \begin{tabular}{c|c|c|c|c|c|c|ccc}
%         \toprule
%         \multirow{2}{*}{Method} & \multirow{2}{*}{Params} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{\makecell{Backbone Pre-training \\ Dataset }} &  \multirow{2}{*}{\makecell{Detection Pre-training \\ Dataset }}   & \multicolumn{2}{c|}{{ val}} & \multicolumn{2}{c}{{test}} \\
%         & & &  && \scriptsize w/o TTA& \scriptsize w/ TTA &\scriptsize w/o TTA&\scriptsize w/ TTA \\
%         \midrule
%         \multicolumn{5}{c}{{\textbf{Instance segmentation on COCO}}}&\multicolumn{4}{c}{AP} \\
%         \midrule
%         % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
%         Mask2Former~\cite{cheng2021mask2former} & $216$M & SwinL & IN-22K-14M & -    & $50.1$ & $-$ & $50.4$ & $-$ \\
%         Soft Teacher~\cite{xu2021end} & $284$M & SwinL & IN-22K-14M & O365     &$51.9$ & $52.5$ & $-$ & $53.0$ \\
%         SwinV2-G-HTC++~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & O365    & $53.4$ & $53.7$ & $-$ & $54.5$\\
%         \hline
%         MasK DINO(Ours) & $\textbf{223}${M} & SwinL & IN-22K-14M & O365 &    $\textbf{54.5}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.1)} & $\textbf{-}$ & $\textbf{-}$ & $\textbf{-}$ \\
%         \midrule
%         \multicolumn{5}{c}{{\textbf{Panoptic segmentation on COCO}}}&\multicolumn{4}{c}{PQ} \\
%         \midrule
%         % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
       
%         Panoptic SegFormer~\cite{li2021panoptic}& $-$M & SwinL & IN-22K-14M & -     &$55.8$ & $-$ & $56.2$ & $-$ \\
%          Mask2Former~\cite{cheng2021mask2former} & $216$M & SwinL & IN-22K-14M & -     & $57.8$ & $-$ & $58.3$ & $-$ \\
%         % SwinV2-G~\cite{liu2021swinv2} & $3.0$B & IN-22K-ext-70M~\cite{liu2021swinv2} & O365 &   & $61.9$ & $62.5$ & $-$ & $63.1$\\
%         \hline
%         MasK DINO (ours) & ${223}$\textbf{M} & SwinL & IN-22K-14M & O365 &    $\textbf{59.4}$\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.6)} & $\textbf{-}$ & $\textbf{-}$ & $\textbf{-}$ \\
%         \midrule
%         \multicolumn{5}{c}{{\textbf{Semantic segmentation on ADE20K}}}&\multicolumn{4}{c}{mIoU} \\
%         \midrule
%         % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
%         Mask2Former~\cite{cheng2021mask2former} & $215$M & SwinL & IN-22K-14M  & -     & $56.1$ & $57.3$ & $-$ & $57.3$ \\
%         Mask2Former~\cite{cheng2021mask2former} & $217$M & SwinL-FaPN & IN-22K-14M  & -     & $56.4$ & $57.7$ & $56.4$ & $57.7$ \\
%         SeMask-L MSFaPN-Mask2Former~\cite{jain2021semask} & $-$M & SwinL-FaPN & IN-22K-14M & -     &$-$ & $58.2$ & $-$ & $58.2$ \\
%         SwinV2-G-UperNet~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & - &    $-$ & $-$ & $59.3$ & $59.9$\\
%         \hline
%         MasK DINO (ours) & $\textbf{223}$\textbf{M} & SwinL & IN-22K-14M & O365 &    $\textbf{59.3}$ & $\textbf{60.3}$ & $\textbf{-}$ & $\textbf{-}$ \\
%         \bottomrule
%     \end{tabular}
%     \end{adjustbox}
%     % }
%     % \vspace{0.05cm}
%     \caption{Comparison of the SOTA models on three segmentation tasks. We outperform all existing models. 
%     % Similar to DETR~\cite{carion2020end}, we use the term ``end-to-end'' to indicate if a model is free from hand-crafted components like RPN and NMS.
%     ``O365''  denotes the  Objects365~\cite{shao2019objects365} dataset. 
%     }
%     \label{tab:sota}
%     % \vspace{-.6cm}
% \end{table}

==> resources/tables/trivial_extend.tex <==
\begin{table*}[t]
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{minipage}[t]{0.55\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|ccc}
    \toprule
    Model & Box AP & Mask AP  \\
        \midrule
        Mask2Former & ${46.2}^*$ & $43.7$     \\
        \midrule
        Mask2Former + detection head&${21.6}$&$41.3$\\
        \midrule
     DINO     &$\textbf{50.7}$    & $-$  \\
    
    \bottomrule
\end{tabular}
\caption{Simply adding a detection head to Mask2Former results in low detection performance. $^*$ indicates the boxes are generated from the predicted masks. The generated boxes from Mask2Former are also inferior to DINO (-4.5)AP. The models are trained for 50 epochs.
}
\label{tab:mask2former_head}
\end{minipage}\hspace{3mm}

\begin{minipage}[t]{0.65\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|ccc}
    \toprule
    Model & Box AP & Mask AP  \\
        \midrule
        DINO + Mask2Former segmentation head&${49.9}$&$40.2$\\
        \midrule
     \begin{tabular}[c]{@{}c@{}}DINO + DETR segmentation head \\(finetune DINO pretrained on COCO detection)\end{tabular}      &${-}$    & $35.8$  \\
     \midrule
     Mask2Former &$-$ &$\textbf{43.7}$ \\
    \bottomrule
\end{tabular}
\caption{Simply adding a segmentation head to DINO results in low instance segmentation performance.  The predicted masks from Mask2Former are also inferior to Mask2Former (-3.5)AP. The models are trained for 50 epochs.
}
\label{tab:dino_head}
\end{minipage}\hspace{3mm}

% \begin{minipage}[t]{0.55\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% \begin{tabular}{c|ccc}
%     \toprule
%     Model & Box AP & Mask AP  \\
%         \midrule
%         DINO + Mask2Former segmentation head&${49.9}$&$40.2$\\
%         \midrule
%      DINO + DETR segmentation head ((finetune DINO pretrained on COCO detection))     &${-}$    & $35.8$  \\
%      Mask2Former &$-$&$43.7$
    
%     \bottomrule
% \end{tabular}
% \caption{Simply adding a segmentation head to DINO results in low segmentation performance.  
% }
% \label{tab:mask2former_head}
% \end{minipage}\hspace{3mm}


% % \vspace{-5.5pt}
% \begin{minipage}[t]{0.42\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% % \vspace{-30.5pt}
% \begin{tabular}{c|ccc}
%     \toprule
%   Feature scale & box AP & {mask AP}  \\
%         \midrule
%     single scale(1/8)     &  $45.8$    & $45.1$  \\
%      3 scales  & $50.5$ & $45.8$   \\
%     4 scales & $50.5$ & $\textbf{46.0}$     \\
%     \bottomrule
% \end{tabular}
% \caption{Comparison of multi-scale features for Transformer decoder under the 50-epoch setting. Both detection and segmentation benefit from more feature scales.}
% \label{tab:feature_scale}
% \end{minipage}\hspace{3mm}
% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \centering
% % \vspace{-31pt}
% \begin{tabular}{c|ccc}
%     \toprule
%   Decoder layer\# & Box AP & {Mask AP}  \\
%         \midrule
%         3&$43.1$&$40.7$\\
%      6     &$44.3$    & $41.1$  \\
%      9  &  $44.5$    & $\textbf{41.4}$  \\
%     12 & $44.8$ & $41.1$     \\
    
%     \bottomrule
% \end{tabular}
% \caption{Decoder layer number comparison under the 12-epoch setting. Mask DINO benefits from more decoders, while DINO's performance will decrease with 9 decoders.}
% \label{tab:dec_layer}
% \end{minipage}

\end{adjustbox}
\vspace{-.4cm}
\end{table*}


